AttriBoT: A Bag of Tricks for Efficiently Approximating Leave-One-Out Context Attribution

The influence of contextual input on the behavior of large language models (LLMs) has prompted the development of context attribution methods that aim to quantify each context span's effect on an LLM's generations. The leave-one-out (LOO) error, which measures the change in the likelihood of the LLM's response when a given span of the context is removed, provides a principled way to perform context attribution, but can be prohibitively expensive to compute for large models. In this work, we introduce AttriBoT, a series of novel techniques for efficiently computing an approximation of the LOO error for context attribution. Specifically, AttriBoT uses cached activations to avoid redundant operations, performs hierarchical attribution to reduce computation, and emulates the behavior of large target models with smaller proxy models. Taken together, AttriBoT can provide a >300x speedup while remaining more faithful to a target model's LOO error than prior context attribution methods. This stark increase in performance makes computing context attributions for a given response 30x faster than generating the response itself, empowering real-world applications that require computing attributions at scale. We release a user-friendly and efficient implementation of AttriBoT to enable efficient LLM interpretability as well as encourage future development of efficient context attribution methods.

==> archive/Experiment_Setup.tex <==
\section{Experimental Setup} \label{sec:experimental_setup}

\subsection{Baselines}

\begin{itemize}[leftmargin=*]
    \setlength\itemsep{0em}
    \item Attention weights: One way to interpret language models is through its attention weights. To compute how each individual source is attended when generating the response, we summed the average attention weights of the source's individual tokens across all heads in every layer when generating the response tokens.
    \item Gradient norm: \cite{yin2022interpretinglanguagemodelscontrastive} \fy{TODO}
    \item Semantic similarity with sentence embedding: We utilized a pretrained embedding model (all-MiniLM-L6-v2) \cite{SentenceBERT} to compute the semantic similarity between the generated response and each one of the sources as the attribution score. 
    \item ContextCite: By randomly ablating a specific portion (for example half) of the sources in context each time, ContextCite learns a linear surrogate model and treats the weights as the attribution scores to approximate LOO. \cite{ContextCite}
\end{itemize}


\subsection{Datasets}

\fy{Add data preprocess/filter steps}

Be upfront about how there are other applications of context attribution but we focus on open-book QA because it provides a realisitc and well-defined way to test out our context attribution method (reviewers will probably ask for other settings).

\begin{itemize}[leftmargin=*]
    \setlength\itemsep{0em}
    \item SQuAD2.0 \cite{squadv2}: Stanford Question Answering Dataset (SQuAD) is a reading comprehension dataset based on Wikipedia articles. 
    \item HotpotQA \cite{yang2018hotpotqa}: HotpotQA is a mulit-hop question answering dataset which requires the system to reason across different sources (Wikipedia paragraphs) and exclude similar but unrelated sources. 
    \item QASPER \cite{qasper}: QASPER is a document-grounded, information-seeking question answering dataset where each context is a natural language processing papaer. 
\end{itemize}

\subsection{Models}

We used the instruction tuned models from the Llama 3.1 family \cite{dubey2024llama3herdmodels} and the Qwen 2.5 family \cite{qwen2}.

\fy{Add stuffs like 8B, 70B. TODO: Llama to Qwen is working but not Qwen to Llama. Fix Llama 3 citation.}


% -Datasets
%     -SQuAD
%     -Hotpot QA
%     -Qasper
%     -Some notes on how each are pre-processed/filtered
% -Models
%     -Llama-3.1 70B and 8B
%     -QWEN2.5
% -Evaluation Metrics (perhaps this belongs in Problem Statement section)
%     -Introduce ESD test for determining number of outliers
%     -Top-k-intersection
%     -Top-k RBO

==> archive/Introduction.tex <==
\section{Introduction} \label{sec:introduction}

% Is it OK to follow how ContextCite write their paper? We don't really have difference in problem settings.

% Motivate the problem
% -What is context attribution?
%\fy{One survey paper: https://github.com/HITsz-TMG/awesome-llm-attributions . Currenlty most attribution methods rely on LLM itself (CoT, verification), still issues about Hallucination, bias, knowledge conflict, etc.}
%Recent retrieve-augmented generation (RAG) techniques have demonstrated the strong capabilities in improving the response quality from large language models (LLM) \cite{RetrievalQA} \cite{RAGTrillionTokens}, reduce Hallucination \cite{RAGHallucination}
% Context attribution: (contributive) interpret the value (importance) of a source for a generated response.

% Goal: emphasize context attribution is very important
% -Why is it necessary, how is it currently applied?
% Possible application, practical applications and audiences: 
% - Interpreting the response
% - Value provided source
% - (Hallucination detection, source?)
% - (Improve correctness, not really?)
% - Detecting poisoned attacks
% Need references for these. 

% Goal: emphasize although context attribution is important, efficiency and interpretability restricts people to use it.
% -What are the difficulties preventing people from doing this (efficiency)? 
% -What are the shortcomings of current approaches to this problem?
% Current approcach: 
% - LOO, great interpretation, very low efficiency, infeasible to compute for long context, $O(N^2)$?
% - ContextCite: multiple rounds of inference, still high cost
% - Citations: not interpretable
% - Attention weights: still controversy in terms of interpretability
% - Similarity: not helpful for multihop, or short responses
% May need to get the EMR back to demonstrate if we are providing higher accuracy?

% Goal: demonstrate that we solve the issue, and brought some other insight
% -What are our contributions at a high-level.
% Contributions:
% - Bag of tricks: kv-cache, hierarchical, pruning, proxy (this as our novelty?)
% - Pareto optimal performance: feasible for real world applications
% - When same response provided, same model family establishes similar behavior
% - Clean api

The proliferation of large language models (LLMs) has rapidly increased in recent years -- for example, the integration of OpenAI's GPT-4 \cite{openai2024gpt4technicalreport} and Google's Gemini \cite{geminiteam2024geminifamilyhighlycapable} in Apple and Android-based products has put them in the hands of billions of users.
As LLMs become more widely used, the consequences of incorrect or problematic outputs will continue to grow along with their influence on information access, decision-making, and social interactions.
The risks and impact of this widespread adoption spurs the need for a deeper understanding of how LLMs generate their outputs.
Indeed, a great deal of recent work on LLM interpretability aims to uncover and elucidate their inner workings, including determining the influence of pre-training data \citep{} and mechanistically understanding their underlying architecture \citep{}.

A key usage pattern for LLMs involves feeding in contextual information as part of their input.
For example, in retrieval-augmented generation (RAG) \citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}, documents from an external datastore that are relevant to a given query are retrieved and fed into the model's input.
This allows LLMs to process data or make decisions based on information that is not available in their pre-training dataset, which has proven critical to making LLMs applicable to a wide range of use cases.
While inspecting the documents retrieved by a RAG system can provide a form of interpretability, LLMs generally provide no direct insight into which part of the augmented context influenced the model's generation. 
This lack of transparency hinders practitioners' abilities to verify model responses as well as to assign credit to informative sources.
To address this shortcoming, \textit{context attribution} methods \citep{} aim to quantify the influence of each span of text in an LLM's context.

A natural approach for context attribution is to remove a given span of text from the context and measure the ensuing change in the likelihood of the model's original response. 
This notion of importance, known as the Leave-One-Out (LOO) error, is a common notion used in training data attribution \citep{koh2020understandingblackboxpredictionsinfluence}, data valuation \citep{choe2024dataworthgptllmscale}, feature attribution \citep{li2017understandingneuralnetworksrepresentation}, and recently has been explored for context attribution \citep{cohenwang2024contextciteattributingmodelgeneration}. 
While the LOO error produces meaningful and interpretable context attribution scores, it is often viewed as impractical due to the need to to perform an independent forward pass to score each text span in the context. 
This is particularly problematic for modern LLMs where forward passes are computationally expensive and realistic use cases often have long contexts with many text spans (e.g., sentences or paragraphs) to score.

% While the LOO error yields meaningful and interpretable scores, it is often 

%In this work, we propose and evaluate a suite of methods for efficiently approximating LOO attributions. Specifically, we design methods that leverage key-value caching, source pruning to avoid scoring spans that are unlikely to contain high-value text, and smaller proxy LMs, all of which when composed achieve a $\sim100\times$ speedup over naively computing LOO attributions. Furthermore, we find that these methods ... something something pareto optima
%In this work, we propose and evaluate a suite of methods for making LOO attribution tractable at LLM scale. First, we find that approximately half of the FLOPs used to naively compute LOO attributions are redundant and can be avoided by caching the attention key and value tensors at each layer  \citep{pope2022efficientlyscalingtransformerinference}. Second, we observe that the sum of $k$ LOO attributions are well-approximated by a single Leave-$k$-Out attribution score, allowing us to remove large sections of unimportant text at a coarse level before scoring individual fine-grained sources. Finally, we find that the LOO attribution scores for large (e.g., 70B parameter) models are often similar to smaller (e.g., 8B parameter) models from the same model family. This allows us to prune sources that are likely to be low-attribution based on the scores of a small model, or to simply use a small model in place of a larger model of interest.


% In this work, we propose and evaluate a suite of methods for making LOO attribution tractable at LLM scale. We test our 

In this work, we aim to show that LOO context attributions can be efficiently approximated at LLM scale.
To do so, we leverage the following observations:
\begin{enumerate}[leftmargin=*]
    \item Approximately half of the FLOPs needed to na\"ively compute LOO attributions are redundant and can be avoided by caching the attention key and value tensors at each layer  \citep{pope2022efficientlyscalingtransformerinference}.
    \item The sum of the LOO attributions for $k$ contiguous text spans (e.g., sentences in a paragraph or paragraphs in a section) are well-approximated by a single Leave-$k$-Out attribution score.
    \item The LOO attribution scores for a large model (e.g., 70B parameters) are well-approximated by smaller models (e.g., 8B parameters) in the same model family.
\end{enumerate}

%Leveraging these findings, we design a set of approximate LOO attribution methods that trade off attribution speed with approximation error.
These findings naturally lend themselves to novel efficient key-value caching schemes, hierarchical approaches that remove low-information paragraphs before attributing at the sentence-level, and the use of smaller proxy LMs to approximate the LOO behavior of a larger target model.
We develop and explore the practical application of these schemes to develop an aggregate system called AttriBoT (a \textbf{B}ag \textbf{o}f \textbf{T}ricks for efficient context attribution).
When evaluating AttriBoT in the open-book question answering setting (where a model is presented a question with one or more related documents provided in its context), we find that our methods significantly reduce the cost of computing LOO attributions -- at times by \textgt$100\times$ -- while remaining more faithful to the orignal model's LOO error than a wide range of baselines.
In addition, the cascade of approaches underlying AttriBoT can be naturally modified or ablated to attain a pareto-optimal trade-off between efficiency and accuracy. 
To enable better intepretability of context-augmented LLMs and facilitate future work on context attribution, we release an efficient and user-friendly implementation of AttriBoT.\footnote{\url{https://see-supplementary.com}}

% These outline paragraphs are always superfluous so we can remove it if needed
In the following section, we formalize the problem of context attribution, define the LOO error in detail, and discuss the metrics we use to evaluate a given method's faithfulness.
Then, in \cref{sec:methods}, we detail our novel techniques for speeding up and approximating LOO error, ultimately producing AttriBoT.
Experimental results across multiple model families and datasets are provided in \cref{sec:experimental_setup}, with related work in \cref{sec:related_work} and a conclusion in \cref{sec:conclusion}.


% Ultimately, when compared to several context attribution baselines such as semantic embedding similarity \citep{reimers2019sentencebertsentenceembeddingsusing}, input gradient norms \citep{yin2022interpretinglanguagemodelscontrastive}, attention weights \citep{TODO}, and ContextCite \citep{cohenwang2024contextciteattributingmodelgeneration}, our methods are Pareto optimal over a wide range of efficiencies.
 
% To evaluate how well each method approximates true LOO attributions, we generate responses with a target model and compute ground truth LOO attributions. Using these scores, we identify sentences with outlyingly large attribution scores using the Extreme Studentized Deviate (ESD) statistical test \citep{2e6b5217-1119-3bfe-8b9c-c1af48fb0291}.
% We then compare the approximate LOO attributions produced by each method, by measuring how well they reflect the LOO scores of the original model

%We find that our methods significantly reduce the cost of computing LOO attributions, at times achieving speedups of up to $50\times$ while retaining a mean Average Precision of TODO. 
%Furthermore, these methods can be varied to adjust the tradeoff between speed and accuracy, with all of the methods being Pareto optimal with respect to several baseline context attribution methods.






==> archive/Methods.tex <==
\section{Approximate LOO Attribution Methods} \label{sec:methods}
% -KV caching
% -Hierarchical attribution
% -Pruning
% -Proxy modeling
% -Combination

\subsection{Key-Value Caching}
For a context containing $|C|$ sources, computing $\tau_{LOO}$ requires $|C| + 1$ forward passes. 
However, much of this computation is redundant when the underlying language model is an autoregressive transformer. 

At each self-attention layer in an autoregressive transformer, the key and value tensors at each position in the sequence are a function of only previous tokens due to autoregressive masking \citep{vaswani2023attentionneed}. 
Thus, if two token sequences share a prefix, the key and value tensors for each position in that prefix will be identical for forward passes on both sequences. 
This redundant computation can be avoided by caching the key and value tensors at each layer and reusing the cached values for sequences that have a previously computed prefix \citep{pope2022efficientlyscalingtransformerinference}.

When computing LOO attributions, the keys and values can be cached for the full sequence of tokens while computing $p_{\theta}(R | Q,C)$. 
Then for each subsequent forward pass computing $p_{\theta}(R|Q, C \setminus \{s_i\})$, the cached keys and values for $Q$ and the first $i-1$ sources in $C$ can be reused. 
In aggregate over all sources, this approximately saves half of the FLOPs used to compute $\tau_{LOO}$, as reported in \Cref{tab:theoretical_flops} (see \Cref{appendix} for derivation).

\subsection{Hierarchical Attribution}

\subsection{Proxy Model Attribution}

\subsection{Proxy Model Pruned Attribution}

\subsection{Proxy Model Hierarchical Attribution}

==> archive/Problem_Statement.tex <==
\section{Problem Statement}
% Formally define the problem
% Formally define LOO in autoregressive model, probability to generate the original response, why this is interpretable, why this should be the ground truth?

% -The goal is approximate the LOO attributions
% -What are LOO attributions?

% Independence of attribution, grouped vs individual

\fy{I'm thinking about changing it from context attribution to souce attribtuion? The written is using ContextCite as a reference, so make sure I'm not copying}

We start with introducing leave-one-out context attribution in the setting of autoregressive models, then we will introduce how context attribution acts as an interpretation method. We will also introduce possible applications of context attribution, and why leave-one-out context attribtuion is low efficiency.

% Autoregressive model, log-probability of generating the response
\subsection{Context Attribution in Autoregressive Models}

In an autoregressive language model, every output is a probability distribution given the sequence of past tokens. We express the probability of generating the token $t_{n+1}$ given the previous tokens $t_1, t_2, \ldots, t_i$ as: $P_{LM}(t_{i+1} | t_1, t_2, \ldots, t_i)$. 


To utilize large language models towards performing desired tasks, prompting is applied to instruct the language model. In typical question-answering (QA) setting, the question $Q$ is passed in with related information context $C$ as the prompt and the response $R$ consists the answer for the question. When the response tokens $R=\{r_1, r_2, \ldots, r_j\}$ is generated given the context tokens $C = \{c_1, c_2, \ldots, c_k\}$ and the query tokens $Q=\{q_1, q_2, \ldots, q_l\}$, the probability of generating the response could be written as $P_{LM}(R | C, Q)=P_{LM}(r_1, r_2, \ldots, r_j | c_1, c_2, \ldots, c_k, q_1, q_2, \ldots, q_l)$. 

Recent advancement of large language models have demonstrated their strong capabilities in various tasks, but remain hard to interpret. One of the key questions people eager to answer is that when LLMs answer a question given the context, to what extent the models are using the provided source, or in other words how each one of the sources are contributing in generating the response. The source could be at any granuality level including documents, paragraphs, sentences, words or even characters. We denote the contribution of the source towards generating the response as context attribution.

Formally, given the context with sources $S = \{s_1, s_2, \ldots, s_n\}$, a query $Q$, a language model $P_{LM}$, and the generated response $R$, context attribution is a mapping from $\mathcal{S}^n$ to $\mathcal{R}^n$ that assigns an contribution score to each of the source $s_i \forall i \in 1, \ldots, n$. 

% LOO

\subsection{Calculating Context Attribution Through Context Removal}

As the attribution score quantitively defines the contribution of every single sources towards generating the response, this is equivalent to measuring the effect of removing the source on generating the original response. Therefore, the attribution score $att_i$ for each source $s_i$ could be defined as the change of probability of generating the original response when the source $s_i$ is removed: $att_i = log(P_{LM})(R \, | \, C, \, Q) - log(P_{LM})(R \, | \, C \, \backslash \, \{s_i\}, \, Q)$. This technique is also referred as leave-one-out (LOO). The attribution score is positive if the including the source will increase the probability of generating the response (positive contribution), and larger attribtuion score indicates the source has a large impact on the response. Finding the sources with high attribution score will reveal the context that is important for the model and the response.

\fy{Mention the sources are linear? Grouped vs Individual? LOO vs shapley? The issue is that if we say its linear, why not just use ContextCite?}

\fy{Add time complexity}

% \subsection{Leave-One-Out as a Inefficient Interpretation Tool}

% Explain the interpretation of context attribution, how it could be possibly used, explain the complexity and so it can't be practically used.

% Leave-one-out provides an intuitive and reliable understanding of how each individual source is contributing to generate the response. Existing methods have applied methods in

==> archive/Problem_Statement_V2.tex <==
\section{Problem Statement} \label{sec:problem_statement}
In this section, we introduce the problem of context attribution (\Cref{ssec:context_attribution}), define one approach to context attribution based on the Leave-One-Out (LOO) error (\Cref{ssec:leave_one_out_attribution}), and define how we evaluate approximation accuracy for approximate LOO attribution methods (\Cref{ssec:evaluating_approximate_loo_attributions}). 

\paragraph{Notation}
Suppose that an autoregressive transformer language model generates a response $R$ conditioned on a query $Q$ and a context $C$. 
For the purposes of this paper, we view a language model with parameters $\theta$ as a function $p_{\theta}(R | Q, C)$ that returns the probability of generating a response given a particular query and context. 
Furthermore, we consider the context to be a list of sources $C = [s_{i}]_{i=1}^{|C|}$, where each source is a piece of text like a sentence, paragraph, or document.  

\subsection{Context Attribution} \label{ssec:context_attribution}
Context attribution, first introduced by \cite{cohenwang2024contextciteattributingmodelgeneration}, is the problem of attributing a response generated by a language model back to a specific source in the model's context.
Formally, \cite{cohenwang2024contextciteattributingmodelgeneration} define a context attribution method as a function  $\tau(\theta, s_1, ..., s_{|C|})$ that maps a language model $\theta$ and sources $s_i \in C$ to a vector of real-valued scores indicating each source's importance to the model's response.\footnote{The original formulation of context attribution in \cite{cohenwang2024contextciteattributingmodelgeneration} leaves the dependence of $\tau$ on $\theta$ implicit. Since we later introduce algorithms where smaller proxy models are used to approximate the attributions of larger models, we choose to make this dependence explicit in our notation.}

\subsection{Leave-One-Out Attribution} \label{ssec:leave_one_out_attribution}
There are many notions of what makes a source important that each lead to different choices of $\tau$. 
Perhaps the simplest and most interpretable notion of importance is that important sources lead to large drops in the likelihood of the model's response when they are removed from the original context. 
This quantity, often referred to as the Leave-One-Out error, leads to the following choice of context attribution function, which we refer to as the LOO attribution in the rest of the paper.
\begin{align}
    \tau_{LOO}(\theta, s_1, ..., s_{|C|})_i = \log p_{\theta}(R|Q,C) - \log p_{\theta}(R|Q,C \setminus \{s_i\})
\end{align}
In practice, LOO attributions are often impractical to compute as scoring all $|C|$ sources in the context requires $|C| + 1$ forward passes of the language model -- one forward pass for computing the likelihood of the response given the full context and $|C|$ forward passes for computing the likelihood with each of the $|C|$ sources individually removed from the context.
For this reason, attributing a response back to contexts containing a large number of sources can be orders of magnitude more expensive than generating the response itself.
Thus, the remainder of this paper explores various methods for efficiently approximating $\tau_{LOO}$.

\subsection{Evaluating Approximate LOO Attributions} \label{ssec:evaluating_approximate_loo_attributions}
\paragraph{Approximation Error}
Past work has found that for domains like summarization and question answering, attributions tend to be sparse, meaning that only a small number of sources in the context influence a model's response \citep{cohenwang2024contextciteattributingmodelgeneration}. Thus, when evaluating how well an attribution algorithm approximates LOO attributions, we primarily care about how well the algorithm recovers these few highly contributive sources.

To evaluate approximate LOO attribution methods we first compute the exact LOO attributions and identify the sources with outlyingly large scores. We do this by applying the Generalized Extreme Studentized Deviate (ESD) test \citep{2e6b5217-1119-3bfe-8b9c-c1af48fb0291}, an iterative statistical test that, given an upper bound on the number of outliers, returns the outlier values in a collection of data. We denote the number of detected outlier sources for a given example as $R$.

We then test the extent to which the approximate LOO attributions recover these $R$ outlier sources using evaluation metrics from information retrieval. In particular, we rank the sources according to their approximate LOO attribution scores and measure the $R$-Precision (equivalent to the Precision@$R$ and Recall@$R$ where $R$ is the number of informative sources) and the mean Average Precision (mAP) \citep{10.5555/1394399}. 

\paragraph{Efficiency}
For each approximate LOO algorithm, we report its practical and theoretical efficiency. To measure practical efficiency, we report both the average GPU-seconds and wall-clock seconds needed to compute attribution scores for all sources in a context. For theoretical efficiency, we estimate the number of floating-point operations (FLOPs) needed to compute attributions as a function of the number of model parameters $P$, the number of sources $|C|$, the number of tokens per source $T$, and any other method-specific parameters. To estimate FLOPs, we use the simplifying assumptions from \cite{kaplan2020scalinglawsneurallanguage} and \cite{hoffmann2022trainingcomputeoptimallargelanguage} that performing a forward pass for a $P$-parameter language model on $D$ tokens requires approximately $2PD$ FLOPs. Based on these assumptions we report estimated FLOP counts in \Cref{tab:theoretical_flops}.

